Automated LTL Specification Generation from Industrial Aerospace Requirements

In the development and verification of safety-critical aero-space software, Linear Temporal Logic (LTL) has been widely used to specify complex system properties derived from requirements. However, a significant gap remains in industrial practice: translating natural language (NL) requirements into formal LTL properties is a labor-intensive and error-prone process that requires rare expertise in both aerospace control engineering and formal methods. While recent NL-to-LTL tools (e.g., NL2SPEC, NL2TL, NL2LTL) are capable of automating parts of this process, they often fail on real requirement documents in industrial settings, due to complex domain terminology or implicit temporal and logical structure. To address these challenges, we present AeroReq2LTL, a framework that automates LTL property generation for aerospace requirements using large language models (LLMs), with two key industrial innovations: (i) a data dictionary that normalizes technical jargon into precise atomic propositions; and (ii) a template-based requirement language that makes temporal cues and logical relations explicit before translation. On a real aerospace dataset, AeroReq2LTL achieves 85% precision and 88% recall in LTL generation, and its outputs can be directly consumed by existing verification tools.

==> Figure/case1.tex <==
%%%% this is minipage(white box)
\begin{figure}[t]
%\vspace{7.5pt}
\centering
\scriptsize
\fbox{%
\begin{minipage}{1\columnwidth}
\raggedright
\vspace{1pt}

\textbf{Input \texttt{Req39}:} In the event that the BeiDou signal is unavailable for a duration exceeding 12.8s while operating in inertial navigation mode, the navigation computer is required to initiate an immediate transition to the star tracker system.

\rule[0pt]{12.2cm}{0.05em}

\textbf{NL2SPEC Output:} $G ((a \& b) \to F c)$
 
Explanation of translation.
1) Globally, we are checking this condition over the entire timeline `G'.
2) a \& b, if the BeiDou signal is unavailable `a' and the system is in inertial navigation mode `b'.
3) F c, eventually, the transition to the star tracker system `c' must occur.

\rule[0pt]{12.2cm}{0.05em}

\textbf{\aero Output:}
\vspace{1pt}

\texttt{TNL39}. In (subMode = INM) the navigation computer shall immediately satisfy if (flagBD = FALSE \& deTCount > 12.8) then (flagSTS = TRUE).
\vspace{1pt}

\texttt{LTL39}. G((subMode = INM $\land$ flagBD = FALSE $\land$ deTCount > 12.8) $\to$ (flagSTS = TRUE)

\end{minipage}}
\setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{-15pt}
\caption{Comparative Analysis of Results from two Methods.}\label{fig:case1}
\end{figure}

==> Figure/nl2tnl.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=0.85\textwidth]{images/Workflow2.pdf}
    \setlength{\abovecaptionskip}{5pt}
    \setlength{\belowcaptionskip}{-15pt}
    \caption{The workflow of \aero NLtoTNL Converter.}
    \label{fig:NLtoTNL}
\end{figure}

==> Figure/spacekg.tex <==
\begin{figure}[t]
\vspace{-5pt}
    \centering
    \includegraphics[width=1\textwidth]{images/Figure2_SpaceKG.pdf}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-15pt}
    \caption{Examples of original requirement statements, corresponding SpaceKG entries, and templated natural language statements.}
    \label{fig:spacekg}
\end{figure}

==> Table/Table2.tex <==
\begin{table*}[t]
\footnotesize
%\vspace{-15pt}
  \centering
    \setlength{\abovecaptionskip}{2.5pt}
    \setlength{\belowcaptionskip}{-7.5pt}
  \caption{Typical examples of requirement description templates. Among these, the State-Change template is the most used, representing a state transition; the Bound-Check template indicates that the system must meet a certain boundary condition; and the Work-Mode-Change template represents a switch in the control system's operational mode. The red content in the requirement templates corresponds to the fillable fields, while the bold content in the TNL statements provides examples of how these fields are populated.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lll}
    \toprule
    \rowcolor[rgb]{ .851,  .851,  .851} \textbf{S No.} & \textbf{Type} & \textbf{Requirement Templates and TNL Statements} \\
    \midrule
    \multirow{2}[2]{*}{1} & State & \textcolor{purple}{\textbf{Component}} shall always satisfy if ( \textcolor{purple}{\textbf{input\_state}} \& \textcolor{purple}{\textbf{condition}}) then next \textcolor{purple}{\textbf{output\_state}}. \\
          & Change   & 
          \textbf{`Communicator'} shall always satisfy if (\textbf{`signal\_lost'} \& \textbf{`mission\_phase'}) then next\textbf{`backup'}.
         \\
    \midrule
    \multirow{2}[2]{*}{2} & Bound & In \textcolor{purple}{\textbf{work\_mode}}, the \textcolor{purple}{\textbf{component}} shall always satisfy \textcolor{purple}{\textbf{bounds}}. \\
          & Check   & In \textbf{`pitch\_search mode'}, the \textbf{`gyroscope'} shall always satisfy \textbf{`roll\_target\_velocity = 0'}. \\
    \midrule
    \multirow{2}[2]{*}{3} & Work Mode & Upon ( \textcolor{purple}{\textbf{input\_work\_mode}} \& \textcolor{purple}{\textbf{condition}} ) \textcolor{purple}{\textbf{component}} shall at the next timepoint satisfy \textcolor{purple}{\textbf{output\_work\_mode}}. \\
          & Change   & Upon ( \textbf{`pitch\_search'} \& \textbf{`sun\_not\_found'} ) \textbf{`Spacecraft'} shall at the next timepoint satisfy \textbf{`roll\_search'}. \\

          % TNL   & Upon ( \textbf{`pitch\_search'} \& \textbf{`mode\_duration'} $\geq$ 720s \& \textbf{`sun\_not\_found'} ) \textbf{`Spacecraft'} shall at the next timepoint satisfy \textbf{`roll\_search'}. \\
    
    \midrule
    \multirow{2}[2]{*}{4} & Command & Upon \textcolor{purple}{\textbf{command}} the \textcolor{purple}{\textbf{component}} shall \textcolor{purple}{\textbf{timing}} satisfy \textcolor{purple}{\textbf{action}}. \\
          & Process   & Upon \textbf{`command\_opcode = 29'} the software shall \textbf{`immediately'} satisfy \textbf{`retract\_landing\_gear\_command'}. \\

          
    \midrule
    \multirow{2}[2]{*}{5} & State & 
    
    In \textcolor{purple}{\textbf{work mode}} the \textcolor{purple}{\textbf{component}} shall immediately satisfy if \textcolor{purple}{\textbf{condition}} then \textcolor{purple}{\textbf{response}}.
    
    \\
          & Response   & In \textbf{roll\_hold mode} the \textbf{`Spacecraft'} shall immediately satisfy if \textbf{`roll\_angle\_up'} then \textbf{`roll\_hold'}. \\


    \midrule
    \multirow{2}[2]{*}{6} & State & The \textcolor{purple}{\textbf{component}} shall maintain \textcolor{purple}{\textbf{state}} unless \textcolor{purple}{\textbf{condition}}. \\
          & Maintenance   & The \textbf{`alarm system'} shall maintain \textbf{`active'} unless \textbf{`system\_disabled'}. \\

    \midrule
    \rowcolor[rgb]{ .851,  .851,  .851} \multirow{1}[1]{*}{7} &$\dots\dots\dots$  &$\dots\dots\dots$
    
    \\
    \bottomrule
    \end{tabular}}
  \label{tab:templates_example}%
\end{table*}

==> Table/Table3.tex <==
\begin{table}[t]
%\vspace{-15pt}
\footnotesize
\setstretch{0.9}
    \centering
    \setlength\tabcolsep{10pt}
    \setlength{\abovecaptionskip}{2.5pt}
    \setlength{\belowcaptionskip}{-7.5pt}
    \caption{Statistics for Requirement Documents Used for Analysis and Testing}
    \begin{tabular}{lccc}
    \toprule
    \rowcolor[rgb]{ .851,  .851,  .851} \textbf{Category} & \begin{tabular}[c]{@{}c@{}}\textbf{Documents}\\ \textbf{Num}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Average}\\ \textbf{Word Count}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Requirement}\\ \textbf{Num}\end{tabular} \\
    \midrule
    Documents for Analysis & 8     & 2891  & 427 \\
    Documents for Testing & 1     & 3446  & 79 \\
    \bottomrule
    \end{tabular}
  \label{tab:doc_statistics}
  \vspace{-5pt}
\end{table}

==> Table/Table4.tex <==
\begin{table}[t]
%\vspace{-15pt}
\footnotesize
 \setstretch{0.8}
  \centering
    \setlength\tabcolsep{12.5pt}
    \setlength{\abovecaptionskip}{2.5pt}
    \setlength{\belowcaptionskip}{5pt}
  \caption{Statistics of Predefined \\spacekg Entities and Requirement Templates}
  
    \begin{tabular}{lcl}
    \toprule
    \rowcolor[rgb]{ .851,  .851,  .851} \textbf{Category} & \multicolumn{1}{p{3.8em}}{\begin{tabular}[c]{@{}c@{}}\textbf{Total}\\ \textbf{Count}\end{tabular}} & \textbf{Detailed Types} \\
    \midrule
    Predefined \spacekg Entities & 407   & \begin{tabular}[c]{@{}c@{}}Variable names,\\ Domain terms, etc.\end{tabular}  \\
    \midrule
    Requirement Templates & 12     & \begin{tabular}[c]{@{}c@{}}State-Change, Bound-Check,\\ Work-Mode-Change, etc.\end{tabular}  \\
    \bottomrule
    \end{tabular}
  \label{tab:kg_statistics}
  \vspace{-10pt}
\end{table}

==> Tex/3-backup.tex <==
\subsection{Overall Workflow}
\label{subsec:workflow}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{images/Workflow1.pdf}
    \caption{Workflow of AeroReq2LTL. Original Req denotes requirements statements, TNL represents templated natural language, and LTL represents linear temporal logic.}
    \label{fig:workflow1}
\end{figure*}



Based on the challenges identified in Section~2, AeroReq2LTL is designed as a domain-integrated framework for automatically translating industrial aerospace requirements into Linear Temporal Logic (LTL) specifications.
The framework is organized as a multi-stage NL-to-LTL workflow commonly adopted in industrial requirement formalization, consisting of context reconstruction, semantic rewriting, and formal synthesis.
Domain knowledge and temporal semantics are explicitly integrated through two key components, \textit{SpaceKG} and \textit{SpaceRDL}, which enable robust interpretation and normalization of aerospace industrial requirements.
Figure~\ref{fig:workflow1} illustrates the overall workflow.

\paragraph{\textbf{Document Context Reconstruction.}}
Industrial aerospace requirements are not presented as isolated sentences, but as structured engineering artifacts in which functional logic is tightly coupled with interface-level specifications.
To accurately preserve the original engineering intent, AeroReq2LTL reconstructs requirement context from PDF documents through a dual-stream extraction process.

First, the framework identifies and extracts \emph{requirement statements} as complete functional paragraphs.
Rather than processing isolated lines or sentences, each requirement paragraph is preserved in its entirety to retain invocation conditions, control dependencies, and surrounding functional context.
These paragraphs constitute the primary translation targets for subsequent semantic rewriting.
Second, AeroReq2LTL extracts \emph{domain knowledge} from interface description tables embedded in the same documents.
These tables provide authoritative engineering metadata, including signal names, variable identifiers, data types, valid value ranges, and explanatory annotations.
Such interface-level artifacts serve as the grounding source for domain semantics.

The integration of requirement paragraphs and interface metadata provides the contextual input for subsequent domain grounding.
These reconstructed artifacts serve as the raw material for constructing SpaceKG.
Through this dual-stream context reconstruction, subsequent semantic rewriting and formalization operate on a grounded engineering representation rather than on ambiguous textual fragments.




% \paragraph{\textbf{Document Context Reconstruction.}}
% Industrial aero-space requirements are not presented as isolated sentences, but as structured document units that combine functional logic descriptions with interface specifications, as illustrated in Fig.~\ref{fig:figure1a}.
% As the first step of the workflow, AeroReq2LTL reconstructs requirement context from PDF-format documents by identifying functional module boundaries, requirement statements, invocation conditions, and associated interface descriptions.

% Concretely, requirement documents are first partitioned into modular description units according to standardized identifiers (e.g., requirement identifiers and interface description sections).
% By traversing the document pages and locating these identifiers, the framework determines the page ranges corresponding to individual functional modules and labels them with module names.
% Within each module, individual requirement statements are then extracted as the primary translation targets.
% In parallel, interface description tables associated with each module are collected as structured contextual artifacts.

% To robustly handle complex document layouts, such as multi-column text and embedded tables, we employ the PDFPlumber toolkit~\cite{Singer-Vine_pdfplumber_2024}.
% Through this process, each requirement is explicitly bound to its functional module and corresponding interface-level information.
% This contextual reconstruction step ensures that subsequent semantic rewriting and formalization operate on well-defined engineering contexts, rather than on isolated textual fragments, and provides a precise structural basis for domain grounding in later stages.



% \paragraph{\textbf{NL-to-TNL Rewriting.}}
% After context reconstruction, natural-language requirements are rewritten into \emph{Templated Natural Language (TNL)}, a structured intermediate representation that makes control and temporal semantics explicit.
% This step bridges informal requirements and formal specifications by instantiating the semantic structure defined by SpaceRDL.

% The rewriting is performed using a large language model under strict structural constraints.
% Rather than generating logic freely, the model operates as a guided semantic parser.
% It grounds domain-specific terms via SpaceKG to extract atomic paradigms, and then selects and instantiates an appropriate requirement template according to the inferred intent.
% Template-level constraints ensure that the resulting TNL is structurally consistent and semantically explicit.

% By enforcing this template-driven rewriting process, AeroReq2LTL eliminates ambiguity caused by implicit temporal assumptions and heterogeneous phrasing.
% The resulting TNL provides a stable semantic interface for subsequent deterministic translation into LTL.


\paragraph{\textbf{NL-to-TNL Rewriting.}}
After context reconstruction, natural-language requirements are rewritten into \emph{Templated Natural Language (TNL)}, a structured intermediate representation that makes control and temporal semantics explicit. 
This step bridges informal requirements and formal specifications by instantiating the semantic structure defined by \textsf{SpaceRDL}.

The rewriting is performed using a large language model (LLM) under strict structural constraints. 
Rather than generating logic freely, the model operates as a guided semantic parser. 
The core of this process is the semantic grounding of domain-specific terms via \textbf{SpaceKG} to extract atomic paradigms. 
The integration of the previously extracted requirement paragraphs and tabular domain knowledge forms the essential foundation for constructing \textbf{SpaceKG}, following a systematic pipeline: 
(i) \textbf{Data Retrieval:} Identifying all candidate requirement statements and interface metadata from the reconstructed context. 
(ii) \textbf{Intelligent Classification:} Utilizing a BERT-based terminology extractor to categorize tokens into domain terms or program variables based on deep semantic features. 
(iii) \textbf{Expert Mapping \& Standardization:} Collaborating with domain experts to map these terms to standardized \textbf{Atomic Paradigms}.

By leveraging this grounded knowledge, the model selects and instantiates an appropriate requirement template according to the inferred intent. 
Template-level constraints ensure that the resulting TNL is structurally consistent and semantically explicit, eliminating ambiguity caused by implicit temporal assumptions and heterogeneous phrasing. 
The resulting TNL provides a stable semantic interface for subsequent deterministic translation into LTL.




\paragraph{\textbf{TNL-to-LTL Converting.}}
Once requirements are normalized into TNL, their translation into LTL no longer involves open-ended reasoning.
Aero-Req2LTL applies deterministic translation rules that map TNL constructs to corresponding LTL operators.
To support extensibility, translation rules are organized in a prompt repository indexed by template type.
The final output consists of syntactically valid LTL specifications accompanied by structured metadata (e.g., component scope), enabling seamless integration with downstream verification tools.


\subsection{SpaceKG: Domain Grounding for Aerospace Requirements}
\label{subsec:spacekg}

\textit{SpaceKG} is the first core domain-specific component of AeroReq2LTL.
It addresses the semantic grounding challenge identified in Section~2, where long and specialized technical expressions in aerospace requirements often encode single, domain-meaningful engineering predicates that are difficult to interpret using text-only approaches.
To support accurate semantic parsing and subsequent formalization, SpaceKG grounds such expressions in interface-level engineering artifacts and normalizes them into concise, unambiguous atomic paradigms.

\paragraph{\textbf{Knowledge Source and Construction.}}
SpaceKG is constructed directly from the \emph{Interface Description} sections embedded in aerospace requirement documents.\wc{Here, SpaceKG comes from Document Context Reconstruction's KI, remember check.}
These sections specify program-level artifacts that are routinely used by engineers, including variable names, data types, valid ranges, operational modes, and explanatory semantics.
Rather than relying on external ontologies or manually curated vocabularies, SpaceKG derives its knowledge from the same interface-level artifacts that connect requirements to implementation, thereby ensuring semantic consistency across requirements, code, and formal specifications.

In practice, variable names are combined with their associated value constraints to form atomic paradigms suitable for formal reasoning.
For example, the empirical constraint ``\textit{the absolute values of the angular rates on all axes are less than $0.15^\circ$/s continuously for 44.8s}'' is normalized into the atomic expression ``$dwCount > 44.8s$'', which preserves the engineering intent while eliminating linguistic redundancy.
Figure~\ref{fig:spacekg} illustrates representative examples of original requirement statements, corresponding SpaceKG entries, and the resulting normalized expressions.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\textwidth]{images/Figure2_SpaceKG.pdf}
    \caption{Examples of original requirement statements, corresponding SpaceKG entries, and normalized atomic paradigms used in templated natural language.}
    \label{fig:spacekg}
\end{figure}

\paragraph{\textbf{Formal Definition.}}
Formally, SpaceKG is defined as a labeled graph $SpaceKG(\bm{V}, \bm{E})$, where $\bm{V}$ is the set of nodes representing domain entities and $\bm{E} \subseteq \bm{V} \times \bm{V}$ is the set of edges representing semantic relationships among them.
Each node $v \in \bm{V}$ is mapped to a semantic class via a function $\tau: \bm{V} \rightarrow \bm{C}$.
The entity classes include domain terms ($c_{dt}$), abbreviations or alternate names ($c_{an}$), program variable names ($c_{vn}$), and concrete values ($c_{nv}$).
The values in $c_{nv}$ encompass not only booleans, integers, and floating-point numbers, but also predefined operational modes such as ``$RDSM$'', indicating the rate-damp work mode.

Edges in SpaceKG are labeled by relationship types $r \in \bm{R}$ and mapped to pairs of entity classes via a function $\rho: \bm{R} \rightarrow \bm{C} \times \bm{C}$.
Two primary relationship types are defined.
The first, $r_a$, captures conditional relationships between program variables and concrete values, such as ``$flagSP = FALSE$'', representing the condition that the sun is not detected.
The second, $r_m$, captures semantic mappings between program variables and domain terms or their aliases; for example, both ``\textit{sun}'' and ``\textit{sunlight}'' map to the variable \texttt{flagSP}.
Notably, in the aerospace domain, a domain term may correspond to a complete sentence rather than a single noun phrase, reflecting the complexity of engineering conventions in industrial requirement documents.

% \paragraph{\textbf{Role in NL-to-TNL Rewriting.}}
% During requirement formalization, SpaceKG serves as the semantic grounding layer that bridges natural-language descriptions and structured requirement representations.
% By integrating SpaceKG entries into prompt templates, the framework guides the large language model to resolve specialized terminology, extract atomic paradigms, and avoid semantic fragmentation caused by inconsistent phrasing.



\subsection{SpaceRDL and TNL: Explicitizing Implicit Temporal Semantics}
\label{subsec:spacerdl}

The second core contribution of AeroReq2LTL is \textit{SpaceRDL}, a structured requirement description language designed to make implicit temporal and logical assumptions explicit in aerospace control requirements.
As discussed in Section~2, industrial aerospace requirements frequently rely on domain conventions—such as control cycles, physical constraints, and work-mode transitions—without explicitly stating temporal operators, which leads to ambiguity in automated formalization.

SpaceRDL is derived from an empirical analysis of real aerospace control requirement documents.
Although requirement statements exhibit diverse surface forms, their underlying semantics consistently reflect the structured and mode-driven nature of spacecraft control systems.
This observation suggests that the apparent linguistic diversity of requirements can be systematically constrained by an explicit semantic structure aligned with the operational logic of aerospace control software.
Accordingly, SpaceRDL provides a domain-driven semantic scaffold upon which heterogeneous natural-language requirements can be normalized and analyzed.

\paragraph{\textbf{SpaceRDL Structure.}}
Based on the above observation, SpaceRDL defines a fixed set of semantic fields that explicitly capture the core elements of aerospace control logic:
\begin{equation*}
\begin{aligned}
    SpaceRDL = \{\text{workmode}, \text{condition}, \text{component}^*, 
    \text{SHALL}^*, \text{timing}^*, \text{action}^*\}.
\end{aligned}
\end{equation*}

Fields marked with an asterisk are mandatory.
The modal verb \texttt{SHALL*} is immutable and enforces declarative requirement expressions.
The \texttt{component*} field specifies the executor of the control action, while the optional \texttt{workmode} field constrains the operational scope under which the requirement applies; if omitted, the requirement is interpreted as globally applicable across all work modes.

The \texttt{timing*} field explicitly encodes temporal intent using a predefined set of keywords such as \textit{immediately}, \textit{next}, \textit{eventually}, \textit{always}, and \textit{until}, which correspond to standard LTL operators.
The \texttt{condition} field captures either trigger or sustaining semantics and supports logical composition through conjunctions and disjunctions.
By enforcing these structural constraints, SpaceRDL prevents implicit temporal premises from being silently omitted during formalization.

\paragraph{\textbf{Templated Natural Language}}(TNL).
Instantiating the fields of SpaceRDL yields TNL, an intermediate representation that preserves human readability while making control semantics explicit and structured.
Rather than treating requirements as free-form text, TNL constrains each requirement to conform to a predefined semantic template derived from SpaceRDL.

Empirical analysis further shows that the majority of aerospace industrial requirements can be categorized into a limited number of recurring semantic patterns.
These patterns correspond to fundamental control behaviors—such as state transitions, work-mode switches, boundary enforcement, command processing, and conditional responses—and form the basis of a compact template library.
Representative SpaceRDL templates and example TNL instantiations are summarized in Table~\ref{tab:templates_example}.

By enforcing this template-based structure, TNL serves as a semantic contract between informal natural-language requirements and subsequent formal LTL specifications, substantially reducing ambiguity caused by implicit temporal assumptions and heterogeneous phrasing.

% \paragraph{\textbf{Role in NL-to-TNL Rewriting.}}
% A LLM is used as a constrained semantic aligner to map free-form requirements into TNL.
% Its output space is bounded by SpaceRDL templates, while lexical grounding is anchored in SpaceKG.
% The model selects an appropriate template and instantiates its fields with SpaceKG-grounded atomic paradigms, making temporal scope and logical structure explicit.
% As a result, TNL forms a normalized and checkable semantic interface that enables deterministic translation into LTL.








\begin{table*}[t]
  \centering
  \caption{Representative SpaceRDL requirement templates and example TNL instantiations abstracted from aerospace industrial requirements.}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lll}
    \toprule
    \rowcolor[rgb]{ .851,  .851,  .851} \textbf{S No.} & \textbf{Type} & \textbf{Requirement Templates and TNL Statements} \\
    \midrule
    \multirow{2}[2]{*}{1} & State & \textcolor{purple}{\textbf{Component}} shall always satisfy if ( \textcolor{purple}{\textbf{input\_state}} \& \textcolor{purple}{\textbf{condition}}) then next \textcolor{purple}{\textbf{output\_state}}. \\
          & Change   & 
          \textbf{`Communicator'} shall always satisfy if (\textbf{`signal\_lost'} \& \textbf{`mission\_phase'}) then next\textbf{`backup'}.
         \\
    \midrule
    \multirow{2}[2]{*}{2} & Bound & In \textcolor{purple}{\textbf{work\_mode}}, the \textcolor{purple}{\textbf{component}} shall always satisfy \textcolor{purple}{\textbf{bounds}}. \\
          & Check   & In \textbf{`pitch\_search mode'}, the \textbf{`gyroscope'} shall always satisfy \textbf{`roll\_target\_velocity = 0'}. \\
    \midrule
    \multirow{2}[2]{*}{3} & Work Mode & Upon ( \textcolor{purple}{\textbf{input\_work\_mode}} \& \textcolor{purple}{\textbf{condition}} ) \textcolor{purple}{\textbf{component}} shall at the next timepoint satisfy \textcolor{purple}{\textbf{output\_work\_mode}}. \\
          & Change   & Upon ( \textbf{`pitch\_search'} \& \textbf{`sun\_not\_found'} ) \textbf{`Spacecraft'} shall at the next timepoint satisfy \textbf{`roll\_search'}. \\

          % TNL   & Upon ( \textbf{`pitch\_search'} \& \textbf{`mode\_duration'} $\geq$ 720s \& \textbf{`sun\_not\_found'} ) \textbf{`Spacecraft'} shall at the next timepoint satisfy \textbf{`roll\_search'}. \\
    
    \midrule
    \multirow{2}[2]{*}{4} & Command & Upon \textcolor{purple}{\textbf{command}} the \textcolor{purple}{\textbf{component}} shall \textcolor{purple}{\textbf{timing}} satisfy \textcolor{purple}{\textbf{action}}. \\
          & Process   & Upon \textbf{`command\_opcode = 29'} the software shall \textbf{`immediately'} satisfy \textbf{`retract\_landing\_gear\_command'}. \\

          
    \midrule
    \multirow{2}[2]{*}{5} & State & 
    
    In \textcolor{purple}{\textbf{work mode}} the \textcolor{purple}{\textbf{component}} shall immediately satisfy if \textcolor{purple}{\textbf{condition}} then \textcolor{purple}{\textbf{response}}.
    
    \\
          & Response   & In \textbf{roll\_hold mode} the \textbf{`Spacecraft'} shall immediately satisfy if \textbf{`roll\_angle\_up'} then \textbf{`roll\_hold'}. \\


    \midrule
    \multirow{2}[2]{*}{6} & State & The \textcolor{purple}{\textbf{component}} shall maintain \textcolor{purple}{\textbf{state}} unless \textcolor{purple}{\textbf{condition}}. \\
          & Maintenance   & The \textbf{`alarm system'} shall maintain \textbf{`active'} unless \textbf{`system\_disabled'}. \\

    \midrule
    \rowcolor[rgb]{ .851,  .851,  .851} \multirow{1}[1]{*}{7} &$\dots\dots\dots$  &$\dots\dots\dots$
    
    \\
    \bottomrule
    \end{tabular}}
  \label{tab:templates_example}%
\end{table*}




































% To automatically generate LTL specifications for formal verification from the requirement description documents of aerospace control software, we combine domain knowledge, large language models, and formal methods to establish the \textbf{AeroReq2LTL} workflow, as shown in Fig.~\ref{fig:workflow1}.


% \subsection{Original Information Extractor}
% The Original Information Extractor is the data preprocessing component of \textbf{AeroReq2LTL}. It inputs PDF-format requirement documents, intending to filter out translation targets and domain knowledge from the PDF files.


% Aerospace requirement documents follow standardized writing guidelines and are structured based on software functional modules. A single document can be divided into multiple description subunits, similar to Fig.\ref{fig:figure1a}, which facilitates the design of automated processes for batch processing of requirement documents. Given that requirement documents often contain complex content such as tables and multi-column layouts, we use PDFPlumber Toolkit \cite{Singer-Vine_pdfplumber_2024} to capture the target data from the documents.


% The first output of the Original Information Extractor is the original Req statements. We first define characteristic identifiers (\textit{Requirement Identifier, Interface Description}) that can identify subunits. Then, we traverse all pages and use string matching to determine the page range of each subunit. Next, we label these page ranges using the \textit{Module Name}. Finally, we extract all Req statements from each subunit as the processing objects for subsequent translation steps.


% The second output of the Original Information Extractor is domain knowledge. Initially, we extracted all non-requirement textual descriptions from the documents as contextual background for LLMs. However, due to the sparsity of domain knowledge in the texts, LLMs influenced by extraneous information exhibited erroneous predictions. Therefore, we narrow the scope of the domain knowledge filtering. We target the \textit{Interface Description} information from each functional module and category this information based on table column names. In Section~\ref{ssub: spacekg}, we will use \textit{Variable Name}, \textit{Value Range,} and \textit{Explanation} to construct the atomic paradigm for the data dictionary.

% \subsection{NLtoTNL Converter}
% The NLtoTNL Converter is the most critical component of \textbf{AeroReq2LTL}. It uses a pre-trained large language model as its engine, obtaining requirement statements from the Original Information Extractor and rewriting them into templated natural language.

% In this phase, we develop the aerospace data dictionary \textit{SpaceKG}, which serves as an external knowledge source for LLMs. \textit{SpaceKG} gives LLMs more factual support, improving their accuracy in identifying atomic propositions. 
% We also analyze and summarize the characteristics of aerospace control systems, proposing a structured pattern language called \textit{SpaceRDL}. This language remains within the realm of natural language but is more standardized and includes explicit temporal keywords. 
% Finally, through chain-of-thought reasoning and a few-shot prompting approach, we guide LLMs to select appropriate requirement description templates based on the semantics of the original requirement.

% \subsubsection{\textbf{Space Knowledge Graph}}
% \label{ssub: spacekg}

% To achieve accurate natural language parsing, the descriptive phrases of atomic propositions should be as concise and unambiguous as possible. To this end, we mapped the specialized terms in the actual requirement documents to more concise expressions using the domain knowledge graph \textit{SpaceKG}.
% We use the Interface Description provided in the requirement documents as the data source for this concise expression method. We combine variable names and value ranges to form an atomic paradigm like "$dwCount > 44.8s$" to represent the technical term "\textit{the angular rates on all axes are less than 0.15°/s continuously for 44.8}". An example of the original natural language description, the knowledge graph, and the reconstructed expressions is shown in Fig. \ref{fig:spacekg}. 

% \input{Figure/spacekg}

% Specifically, $SpaceKG(\bm{V}, \bm{E})$ defines the correspondences between term nodes in the aerospace domain, where $\bm{V}$ is the set of nodes representing entities, and $\bm{E} \subseteq \bm{V} \times \bm{V}$ is the set of edges representing relationships between entities. $\bm{V} = \{v_1, v_2, \dots, v_n\}$, with each \(v_i\) representing an entity, and $\bm{E} = \{(v_i, {r_{ij}}, v_j) \mid v_i, v_j \in \bm{V}, r_{ij} \in \bm{R}\}$, where $r_{ij}$ denotes the type of relationship, and $\bm{R}$ is the set of all possible relationships. The function \(\tau: \bm{V} \rightarrow \bm{C}\) maps each node \(\bm{V}\) to a class \(\bm{C}\), where \(c \in \bm{C}\) indicates the category to which each entity belongs. The function \(\rho: \bm{R} \rightarrow \bm{C} \times \bm{C}\) specifies which two categories of entities each type of relationship connects. $SpaceKG$ encompasses four types of entities, where \(c \in \{c_{dt}, c_{an}, c_{vn}, c_{nv}\}\), with \(c_{dt}\) representing domain terms, \(c_{an}\) representing abbreviations or alternate names of the terms, \(c_{vn}\) representing variable names in the code, and \(c_{nv}\) representing the actual numeric values in the code. Notably, the values of \(c_{nv}\) include not only booleans, integers, and floating-point numbers but also predefined work modes such as "$RDSM$" , which means \textit{"in the rate damp work mode".} 

% To comprehensively model the relationships between the aforementioned entities, domain experts have defined two types of relationships in $SpaceKG$, where \( r \in \{r_a, r_m\} \). The first type, \( r_a \), represents the conditional relationship between variable names \( c_{vn} \) and actual values \( c_{av} \) in the code. For instance, ``$flagSP = FALSE$'' means ``\textit{the sun is not available}.'' The second type, \( r_m \), is the mapping relationship between variable names in the code \( c_{vn} \) and domain terms \( c_{dt} \), or domain term abbreviations \( c_{an} \) or alternate names \( c_{an} \), e.g. ``\( \textit{sun} \)'' and ``\( \textit{sunlight} \)'' both represent ``\( \text{flagSP} \).''
% Notably, in the aerospace domain, a domain term \( c_{dt} \) can be a complete sentence, as shown in Fig. \ref{fig:spacekg}.

% In practical applications, we used the aforementioned $SpaceKG$ to guide the rewriting of natural language requirement documents into standardized requirement documents. We combine the predefined $SpaceKG$ with the requirement text using prompt templates and employ chain-of-thought reasoning with a large language model \cite{wei2022chainCoT_ref54} to directly rewrite the original text into standardized text.

% To summary, using $SpaceKG$ to normalize and standardize the original natural language requirement descriptions not only helps accurately comprehend the specific intentions and objectives of the requirements during the formal verification process, but also reduces confusion caused by inconsistent terminology. Additionally, standardized terminology facilitates tracking throughout the entire lifecycle of the requirements, ensuring clear verification from requirement collection to implementation and testing according to the requirements documents.

% \subsubsection{\textbf{Templated Natural Language SpaceRDL}}
% \label{ssub:SpaceRDL}

% \textit{SpaceRDL} is a requirement description template focused on spacecraft control systems, where the control systems perform complex computational tasks in fixed operational modes. It is an extension of FRETish~\cite{FRET}, as defined in equation~(\ref{equ:spacerdl}):

% \begin{equation}
% \small
% \begin{aligned}
%     SpaceRDL = \{&\text{workmode}, \text{condition}, \text{component}^*,
%     \text{SHALL}^*, \text{timing}^*, \text{action}^*\}.
% \end{aligned}
% \label{equ:spacerdl}
% \end{equation} \textit{SpaceRDL} consists of six field members, with asterisks indicating mandatory fields and the remaining fields optional. The field \texttt{SHALL*} is immutable, and only \texttt{SHALL*} can be used as the modal verb in requirement descriptions. We hope that \textit{SpaceRDL} can use declarative sentences to express requirements clearly.

% The field \texttt{component*} represents the specific executor of the \texttt{action*}, such as \textit{"the work mode of Spacecraft"} in Req12-Req16 statements. The field \texttt{workmode} specifies the scope of the component behavior, such as \textit{"rate damp," "pitch search," "roll search," and "cruise sun."} If the field \texttt{workmode} is omitted, it indicates that the component behavior is effective in all work modes. If the work mode is selected, \textit{SpaceRDL} offers three types of temporal descriptions for this mode: before the mode, after the mode, and within the mode. \textit{SpaceRDL} defines six possible values for the field \texttt{timing*}: \textit{"immediately,"} \textit{"next,"} \textit{"at the next point,"} \textit{"eventually,"} \textit{"always,"} and \textit{"until,"} which correspond to the logical operators of LTL: current state (no operator), $X$, $U$, $F$, and $G$, respectively.


% \input{Table/Table2}


% The field \texttt{condition} specifies the prerequisites for the \texttt{component*} to execute the \texttt{action*,} such as \textit{"the sun is not detected"} in Req14 (which can be simplified in the data dictionary to flagSP = FALSE). These conditions can be either trigger conditions or sustaining conditions. The former means the action takes effect when the condition becomes true, while the latter means the action remains valid as long as the condition stays true. Trigger conditions are indicated by words like \textit{"upon,"} \textit{"when,"} \textit{"where,"} or \textit{"if,"} while sustaining conditions are introduced by \textit{"whenever."} Conditions can be combined using the keywords "and (\&)" and "or (||)."

% It is worth noting that during the practical process, we observe that the majority of existing requirement statements fall into a small number of semantic templates. Therefore, based on the \textit{SpaceRDL} rules, we provided 12 predefined requirement templates in AreoReq2LTL. Table~\ref{tab:templates_example} presents the six most frequently used semantic templates along with the corresponding TNL statements. In addition, we allow users to create new semantic templates according to the \textit{SpaceRDL} rules, requiring only that the translation rules for the new template be added to the prompt. In Section~\ref{sec:subSpaceRDL}, we will provide a detailed discussion on the usage of semantic templates.

% \input{Figure/nl2tnl}


% \subsubsection{\textbf{Prompt LLM to Rewrite NL into TNL}}
% \label{ssub:nl2tnl}
% After obtaining \textit{SpaceKG} and \textit{SpaceRDL}, we constructed a prompting engineering process to guide LLMs in rewriting natural language text into templated natural language (TNL), as illustrated in Fig.~\ref{fig:NLtoTNL}. The prompting engineering process consists of two steps:


% \begin{itemize}
% \item \textbf{Translate specialized terms into variable names and extract conditional expressions based on the node and relationship definitions in \textit{SpaceKG}.} Initially, the LLM identifies and extracts specialized terms and specific values from the original requirement documents, matches these terms with predefined entities in $SpaceKG$, and translates them into program variable names. It also understands the relationships between entities and ultimately converts these into triplet form expressions, such as \((c_{vn}, r_a, c_{av})\). 
% We refer to this triple structure as the \textit{atomic paradigm}.
% Thanks to LLMs' powerful semantic understanding and contextual learning abilities, we only need to provide a few-shot in-context example for the LLM to accurately translate the program variable names and conditional expressions for us.


% \item \textbf{Rewrite the extracted conditional expressions into TNL based on the predefined format of \textit{SpaceRDL}.} In this step, leveraging the widely used chain of thought technique, we first require LLMs to select the appropriate requirement template type based on the semantics of the original requirement. We first require LLMs to select the appropriate requirement template type based on the semantics of the original requirement.
% Then, we instruct LLMs to integrate the extracted \textit{atomic paradigm} into the requirement template while maintaining the logical relationships of the original requirement. Table \ref{tab:templates_example} showcases our designed 0templates and their usage instructions. This information is used as contextual prompts to ensure that LLMs select the appropriate requirement template in the prompting engineering process.

% \end{itemize}




% The example in Listing 1 demonstrates how the NLtoTNL converter rewrites the NL into the TNL using the data dictionary and requirement templates. LLMs consult the data dictionary to simplify terminologies in sections \ding{172}-\ding{175} into four relational triples, then select the appropriate template by parsing the semantics of the original requirement. For Req13, the LLM selects the Work-Mode-Change template. In TNL13, \textit{"subMode = RDMS"} indicates that the spacecraft is currently in rate damping mode; \textit{"dwCount $>$ 44.8s"} means that the three-axis stability state has lasted for at least 44.8 seconds; \textit{"dwModeTime $>$ 128s"} indicates that the current working mode has lasted at least 128 seconds; and \textit{"subMode = PASM"} shows that the next work mode is the pitch search. 
% For Req28, the LLM selects the State-Response template and successfully identifies the global scope. As a result, no working mode is specified in TNL28, indicating that the requirement applies to all modes.
% By comparing Req and TNL, it can be observed that both types of sentences have the same semantics. However, TNL is more standardized and explicit, with conditions and temporal keywords clearly defined.
% %%%% this is minipage(white box)
% % \vspace{0.2cm}
% \begin{center}
% \fbox{%
% \begin{minipage}{0.9\columnwidth}
% \raggedright
% \textbf{Listing 1: Running Example of NLtoTNL Converter.}
% \vspace{0.2cm}

% Req13. If \textcolor{purple}{\ding{172}the absolute values of the angular rates on all axes are less than 0.15°/s continuously for 44.8s} or if \textcolor{blue}{\ding{173}the rate damp mode lasts for 128s}, the work mode of spacecraft switches from \textcolor{ForestGreen}{\ding{174}rate damp} to \textcolor{orange}{\ding{175}pitch search}.
% \vspace{0.1cm}

% TNL13. Upon (\textcolor{ForestGreen}{\ding{174}subMode = RDSM} $\&$ (\textcolor{purple}{\ding{172}dwCount > 44.8s} $||$ \textcolor{blue}{\ding{173}dwModeTime > 128s})) the workmode of spacecraft shall at the next timepoint satisfy  \textcolor{orange}{\ding{175}subMode = PASM}.
% \vspace{0.2cm}

% Req28. Globally, if \textcolor{purple}{\ding{172}the rational flag of inertial navigation module 1 is true}, and \textcolor{blue}{\ding{173}the rational flag of inertial navigation module 2 is true}, then \textcolor{ForestGreen}{\ding{174}angular velocity of the three-axis stabilizer is set to zero}.
% \vspace{0.1cm}

% TNL28. The three-axis stabilizer shall always satisfy if (\textcolor{purple}{\ding{172}flagNav1 = TRUE} $\&$ \textcolor{blue}{\ding{173}flagNav2 = TRUE}) then \textcolor{ForestGreen}{\ding{174}destRate = 0}.

% \end{minipage}}
% \end{center}
% \vspace{0.2cm}
% %%%%%%

% \subsection{TNLtoLTL Converter}
% The TNLtoLTL converter is the final component of \textbf{AeroReq2LTL}. It takes templated natural language from the NLtoTNL converter and transforms it into LTL specifications, outputting the results in JSON format.
% At this stage, we provide the LLMs with two parts of prompt information. The first part explains the specification of LTL specification, as we expect the LLMs to first understand the mathematical definitions and logical symbols of LTL. Considering the example in Listing 1, there are some intuitive correspondences between TNL and LTL, which we have summarized into translation rules as the second part of the prompt information.

% Since \textbf{AeroReq2LTL} allows users to add new semantic templates using SpaceRDL, expanding all the information into a single prompt file could cause the model to lose focus or miss key details. Therefore, we created a prompt repository to enhance the scalability of the framework, where each semantic template has its corresponding prompt file stored. Upon receiving a TNL statement, the TNLtoLTL converter selects the appropriate prompt file from the repository based on the template type and then translates the TNL into LTL specifications using the two parts of information contained in the file.



% \begin{equation}
% \small
% \begin{aligned}
%   \text{LTL13: } G((subMode = RDSM &\land (dwCount > 44.8 \lor dwModeTime >  128))\\
%   &\to X(subMode = PASM))).
% \end{aligned}
% \label{equ3}
% \end{equation}

% \begin{equation}
% \small
% \begin{aligned}
%   \text{LTL28: } G((flagNav1 = TRUE  \land  flagNav2 = TRUE ) \to (destRate = 0)).
% \end{aligned}
% \label{equ4}
% \end{equation}
% \vspace{0.5pt}

% Equation (\ref{equ3}) and (\ref{equ4}) show the results of this processing stage. 
% The meaning of LTL13 is that over the entire time series ($G$), as long as the condition on the left holds, the result on the right must be valid at the next time point ($X$). It is worth noting that the natural language describing components is not translated into the formula, as LTL syntax does not directly support such behavior. Therefore, we include the component information involved in each LTL in the final output JSON file. The meaning of LTL28 is that over the entire time series ($G$), as long as the condition on the left holds, the result on the right must be valid in the current state.
